Statistical Consequences of Dueling Bandits

Multi-Armed-Bandit frameworks have often been used by researchers to assess educational interventions, however, recent work has shown that it is more beneficial for a student to provide qualitative feedback through preference elicitation between different alternatives, making a dueling bandits framework more appropriate. In this paper, we explore the statistical quality of data under this framework by comparing traditional uniform sampling to a dueling bandit algorithm and find that dueling bandit algorithms perform well at cumulative regret minimisation, but lead to inflated Type-I error rates and reduced power under certain circumstances. Through these results we provide insight into the challenges and opportunities in using dueling bandit algorithms to run adaptive experiments.

==> Statistical Consequences of Duelling Bandits (Long-Preprint)/algorithm.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Original Source: 

% Wu, H. and Liu, X., 2016. Double thompson sampling for dueling bandits. arXiv preprint arXiv:1604.07101.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[htbp]
\caption{D-TS for Copeland Dueling Bandits}
\label{alg:dts_Copeland}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand\algorithmiccomment[1]{%
{//{\it ~{#1}}}%
}
\begin{algorithmic}[1]
\STATE{\bfseries Init:} $\bs{B} \gets {\bs{0}_{K \times K}}$; \COMMENT{$B_{i j}$ is the number of time-slots that the user prefers arm $i$ to $j$.}
\FOR{$t = 1$ {\bfseries to} $T$}
\STATE{\COMMENT{Phase 1: Choose the first candidate $a^{(1)}$} }     \label{alg_line:first_candidate_start}
     \STATE{$\bs{U} := [u_{ij}]$,   $\bs{L} := [l_{ij}]$, where $u_{ij}= \frac{B_{ij}}{B_{ij} + B_{ji}}+ \sqrt{\frac{\alpha \log t}{B_{ij} + B_{ji}}}$, $l_{ij} =  \frac{B_{ij}}{B_{ij}+ B_{ji}} - \sqrt{\frac{\alpha \log t}{B_{ij}+ B_{ji}}}$, if $i \neq j$, and $u_{ii} = l_{ii} = 1/2$, $\forall i$;}   \COMMENT{$\frac{x}{0} := 1$ for any $x$.}
    \STATE{$\hat{\zeta}_i \gets \frac{1}{K - 1}\sum_{j \neq i} \mathds{1} (u_{ij}> 1/2)$;} \COMMENT{Upper bound of the normalized Copeland score.}
    \STATE{$\mathcal{C} \gets \{ i: \hat{\zeta}_i = \max_{j} \hat{\zeta}_j\}$;}
    \FOR{$i, j = 1, \ldots, K$ with $i < j$ }
             \STATE{Sample $\theta^{(1)}_{ij} \sim {\rm Beta}(B_{ij} + 1, B_{ji}+ 1)$};
             \STATE{$\theta^{(1)}_{ji} \gets 1 - \theta^{(1)}_{ij}$};
    \ENDFOR
   \STATE $a^{(1)} \gets \underset{i \in \mathcal{C} }{\argmax} \sum_{j\neq i} \mathds{1}(\theta^{(1)}_{ij} > 1/2)$;    \COMMENT{Choosing from $\mathcal{C}$ to eliminate likely non-winner arms; Ties are broken randomly.}
\STATE{\COMMENT{Phase 2: Choose the second candidate $a^{(2)}$}}    \label{alg_line:sec_candidate_start}
      \STATE{Sample $\theta^{(2)}_{ i a^{(1)} } \sim {\rm Beta}(B_{i a^{(1)} } + 1, B_{a^{(1)}  i} +1)$ for all $i \neq a^{(1)}$, and let $\theta^{(2)}_{a^{(1)}  a^{(1)} } = 1/2$;  }
      \STATE{$a^{(2)}  \gets \underset{i: l_{i a^{(1)}} \leq 1/2}{\argmax}~ \theta^{(2)}_{i a^{(1)} }$;}
      \COMMENT{Choosing only from uncertain pairs.}
      \label{alg_line:sec_candidate_end}
\STATE{\COMMENT{Compare and Update}}
\STATE{Compare pair $(a^{(1)} , a^{(2)} )$ and observe the result $w$;}
\STATE{Update $\bs{B}$: $B_{a^{(1)} a^{(2)}}\gets B_{a^{(1)} a^{(2)}}+ 1$ if $w = 1$, or  $B_{a^{(2)} a^{(1)}} \gets B_{a^{(2)}a^{(1)}} + 1 $ if $w = 2$;}
\ENDFOR
\end{algorithmic}
\end{algorithm}


==> algorithm.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Original Source: 

% Wu, H. and Liu, X., 2016. Double thompson sampling for dueling bandits. arXiv preprint arXiv:1604.07101.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{algorithm}[htbp]
\caption{D-TS for Copeland Dueling Bandits}
\label{alg:dts_Copeland}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand\algorithmiccomment[1]{%
{//{\it ~{#1}}}%
}
\begin{algorithmic}[1]
\STATE{\bfseries Init:} $\bs{B} \gets {\bs{0}_{K \times K}}$; \COMMENT{$B_{i j}$ is the number of time-slots that the user prefers arm $i$ to $j$.}
\FOR{$t = 1$ {\bfseries to} $T$}
\STATE{\COMMENT{Phase 1: Choose the first candidate $a^{(1)}$} }     \label{alg_line:first_candidate_start}
     \STATE{$\bs{U} := [u_{ij}]$,   $\bs{L} := [l_{ij}]$, where $u_{ij}= \frac{B_{ij}}{B_{ij} + B_{ji}}+ \sqrt{\frac{\alpha \log t}{B_{ij} + B_{ji}}}$, $l_{ij} =  \frac{B_{ij}}{B_{ij}+ B_{ji}} - \sqrt{\frac{\alpha \log t}{B_{ij}+ B_{ji}}}$, if $i \neq j$, and $u_{ii} = l_{ii} = 1/2$, $\forall i$;}   \COMMENT{$\frac{x}{0} := 1$ for any $x$.}
    \STATE{$\hat{\zeta}_i \gets \frac{1}{K - 1}\sum_{j \neq i} \mathds{1} (u_{ij}> 1/2)$;} \COMMENT{Upper bound of the normalized Copeland score.}
    \STATE{$\mathcal{C} \gets \{ i: \hat{\zeta}_i = \max_{j} \hat{\zeta}_j\}$;}
    \FOR{$i, j = 1, \ldots, K$ with $i < j$ }
             \STATE{Sample $\theta^{(1)}_{ij} \sim {\rm Beta}(B_{ij} + 1, B_{ji}+ 1)$};
             \STATE{$\theta^{(1)}_{ji} \gets 1 - \theta^{(1)}_{ij}$};
    \ENDFOR
   \STATE $a^{(1)} \gets \underset{i \in \mathcal{C} }{\argmax} \sum_{j\neq i} \mathds{1}(\theta^{(1)}_{ij} > 1/2)$;    \COMMENT{Choosing from $\mathcal{C}$ to eliminate likely non-winner arms; Ties are broken randomly.}
\STATE{\COMMENT{Phase 2: Choose the second candidate $a^{(2)}$}}    \label{alg_line:sec_candidate_start}
      \STATE{Sample $\theta^{(2)}_{ i a^{(1)} } \sim {\rm Beta}(B_{i a^{(1)} } + 1, B_{a^{(1)}  i} +1)$ for all $i \neq a^{(1)}$, and let $\theta^{(2)}_{a^{(1)}  a^{(1)} } = 1/2$;  }
      \STATE{$a^{(2)}  \gets \underset{i: l_{i a^{(1)}} \leq 1/2}{\argmax}~ \theta^{(2)}_{i a^{(1)} }$;}
      \COMMENT{Choosing only from uncertain pairs.}
      \label{alg_line:sec_candidate_end}
\STATE{\COMMENT{Compare and Update}}
\STATE{Compare pair $(a^{(1)} , a^{(2)} )$ and observe the result $w$;}
\STATE{Update $\bs{B}$: $B_{a^{(1)} a^{(2)}}\gets B_{a^{(1)} a^{(2)}}+ 1$ if $w = 1$, or  $B_{a^{(2)} a^{(1)}} \gets B_{a^{(2)}a^{(1)}} + 1 $ if $w = 2$;}
\ENDFOR
\end{algorithmic}
\end{algorithm}

